$\ell_p$-norm Multiway Cut

We introduce and study $\ell_p$-norm-multiway-cut: the input here is an undirected graph with non-negative edge weights along with $k$ terminals and the goal is to find a partition of the vertex set into $k$ parts each containing exactly one terminal so as to minimize the $\ell_p$-norm of the cut values of the parts. This is a unified generalization of min-sum multiway cut (when $p=1$) and min-max multiway cut (when $p=\infty$), both of which are well-studied classic problems in the graph partitioning literature. We show that $\ell_p$-norm-multiway-cut is NP-hard for constant number of terminals and is NP-hard in planar graphs. On the algorithmic side, we design an $O(\log^2 n)$-approximation for all $p\ge 1$. We also show an integrality gap of $\Omega(k^{1-1/p})$ for a natural convex program and an $O(k^{1-1/p-\epsilon})$-inapproximability for any constant $\epsilon>0$ assuming the small set expansion hypothesis.

==> background.tex <==
\section{Background}
%disconnected example
We note a major difference between min-sum multiway cut and min \lpnormmc: for every $p>1$, the min \lpnormmc of a connected graph could have parts that induce disconnected subgraphs, whereas all parts in the min-sum multiway cut of a connected graph are always connected. To see this, consider the example shown in Figure \ref{fig:disconnected}. In this example, the set of terminals is $\{u_1,v_1,v_2,v_3,v_4\}$, and we set $a=8^{p/(p-1)}$. A multiway cut that groups $u_2$ with one of $v_1,v_2,v_3,v_4$ has $\ell_p$ objective
\[\left((3a+3)^p+3(3a+2)^p+4^p\right)^{\frac{1}{p}},\]
and the multiway cut that groups $u_2$ with $u_1$ has $\ell_p$ objective
\[\left(4(3a+2)^p+8^p\right)^{\frac{1}{p}}.\]
Here the min \lpnormmc is $(\{u_1,u_2\},\{v_1\},\{v_2\},\{v_3\},\{v_4\})$ because


==> hardness-tree.tex <==
\section{NP-hardness on trees}
\begin{theorem}\label{thm:NP-hard}
For every fixed $p>1$, min \lpnormmc is NP-hard on trees.
\end{theorem}
NP-hardness of min-max multiway cut was shown in \cite{ST04} by a reduction from \textsc{3-partition}.
To show NP-hardness of min \lpnormmc, we use a similar reduction from \textsc{3-partition}. \textsc{3-partition} is defined as follows: 

Given a set $S=[3m]$, a sequence of weights $w_1,w_2,\ldots,w_{3m}$, and a bound $B$ satisfying $\sum_{i=1}^{3m}w_i=mB$ and $B/4<w_i<B/2$ for all $i\in[3m]$, the goal is to decide whether there exists a partition of $S$ into $m$ subsets $S_1,S_2,\ldots,S_m$ such that $\sum_{i\in S_j}w_i=B$ for every $j\in[m]$. This problem is known to be NP-hard.

For an instance of \textsc{3-partition} given by a set $S=[3m]$, weights $w_1,w_2,\ldots,w_{3m}$, and bound $B$, we construct an instance of min \lpnormmc as follows. 

To construct $G$, we start with an empty graph, and for each $i\in[3m]$, we add to $G$ a subgraph as shown in Figure \ref{fig:hardness-1}. The edge weights are labelled near the corresponding edges, where $d:=(12m+12)^{\frac{1}{p-1}}$. These $3m$ subgraphs are disjoint from each other. Finally, we add $m$ isolated vertices $t_1,\ldots,t_m$ to $G$. The terminal set is given by $\{x_i^r:i\in[3m],r\in[6]\}\cup\{t_1,\ldots,t_m\}$.
\begin{figure}
    \centering
    \includegraphics[width=0.6\textwidth]{Hardness-2.JPG}
    \caption{The $i$th subgraph in $G$}
    \label{fig:hardness-1}
\end{figure}

We will show that there exists a partition of $S$ into $S_1,\ldots,S_m$ such that $\sum_{i\in S_j}w_i=B$ for each $j\in[m]$ if and only if the min \lpnormmc in $G$ has $\ell_p$ objective at most
\[\left(mB^p+9m(dB)^p+3\sum_{i=1}^{3m}(dB+w_i/3)^p\right)^{1/p}.\]
We start by showing the forward direction.

\begin{claim}
If $S$ can be partitioned into $S_1,\ldots,S_m$ such that $\sum_{i\in S_j}w_i=B$ for each $j\in[m]$, then $G$ has a multiway cut whose $\ell_p$ objective is $\left(mB^p+9m(dB)^p+3\sum_{i=1}^{3m}(dB+w_i/3)^p\right)^{1/p}$.
\end{claim}

\begin{proof}
Consider the multiway cut of $G$ defined by
\[\big\{\{x_i^r\}:i\in[3m],r\in[6]\big\}\cup\big\{\{t_j\}\cup\{v_i:i\in S_j\}:j\in[m]\big\}.\]
The $p$th power of the $\ell_p$-norm objective of this multiway cut is
\[\sum_{j\in[m]}\left(\sum_{i\in S_j}\frac{w_i}{3}\cdot 3\right)^p+3m\cdot 3\cdot(dB)^p+3\sum_{i=1}^{3m}(dB+w_i/3)^p=mB^p+9m(dB)^p+3\sum_{i=1}^{3m}(dB+w_i/3)^p.\]
\end{proof}

For the backward direction, we will start with a structural observation on an optimal multiway cut of $G$.

\begin{claim}
In an optimal multiway cut of $G$ whose $\ell_p$ objective is at most
\[\left(mB^p+9m(dB)^p+3\sum_{i=1}^{3m}(dB+w_i/3)^p\right)^{1/p},\] 
for every $i\in[3m]$, the vertex $v_i$ is in the same part with $t_j$ for some $j\in[m]$.
\end{claim}
\begin{proof}
Consider an optimal multiway cut of $G$ whose $\ell_p$ objective raised to $p$th power is at most $mB^p+9m(dB)^p+3\sum_{i=1}^{3m}(dB+w_i/3)^p$. We will use $X_i^r$ to denote the part containing $x_i^r$ for each $i\in[3m]$ and $r\in[6]$, and $T_j$ to denote the part containing $t_j$ for each $j\in[m]$.

For convenience, we will define $I\subseteq[3m]$ by $I:=\left\{i\in[3m]:v_{i}\in\bigcup_{i'\in[3m],r\in[6]}X_{i'}^r\right\}$.

For every $i\in[3m],r\in[6]$, we have
\[w(\delta(X_i^r))\geq dB+\sum_{i'\in[3m]:v_{i'}\in X_i^r}2w_{i'}/3.\]
We note that if we arbitrarily order the set $\{i'\in[3m]:v_{i'}\in X_i^r\}$ as $\{i_1,\ldots,i_\ell\}$, we have
\begin{align*}
    &\left(dB+\sum_{q=1}^\ell 2w_{i_q}/3\right)^p+(\ell-1)(dB)^p
    \\&\geq \left(dB+\sum_{q=1}^{\ell-1} 2w_{i_q}/3\right)^p+(dB+2w_{i_q}/3)^p+(\ell-2)(dB)^p
    \\&\geq\ldots
    \\&\geq \sum_{q=1}^\ell(dB+2w_{i_q}/3)^p.
\end{align*}
due to convexity.
By repeatedly applying this inequality, we have
\begin{align*}
    \sum_{i\in[3m],r\in[6]}w(\delta(X_i^r))^p
    &\geq \sum_{i\in[3m],r\in[6]}\left(dB+\sum_{i'\in[3m]:v_{i'}\in X_i^r}2w_{i'}/3\right)^p
    \\&\geq \sum_{i\in I}(dB+2w_i/3)^p+(18m-|I|)(dB)^p
    \\&\geq \sum_{i\in I}(dB+B/6)^p+(18m-|I|)(dB)^p
    \\&=|I|(d+1/6)^p B^p+(18m-|I|)(dB)^p.
\end{align*}
Assuming $I\neq\emptyset$, the $p$th power of the $\ell_p$ objective of this multiway cut is at least 
\begin{align*}
    &\sum_{i\in[3m],r\in[6]}w(\delta(X_i^r))^p+\sum_{j=1}^mw(\delta(T_j))^p
    \\&\geq |I|(d+1/6)^p B^p+(18m-|I|)(dB)^p+\sum_{i\notin I}w(\delta(v_i))^p
    \\&=|I|(d+1/6)^p B^p+(18m-|I|)(dB)^p+\sum_{i\notin I}w_i^p
    \\&>|I|(d+1/6)^p B^p+(18m-|I|)(dB)^p+(3m-|I|)(B/4)^p
    \\&=|I|\big((d+1/6)^p-d^p-(1/4)^p\big)B^p+18md^pB^p+3m(1/4)^pB^p.
\end{align*}
Since we assumed the $p$th power of the $\ell_p$ objective of this multiway cut to be at most
\begin{align*}
    mB^p+9m(dB)^p+3\sum_{i=1}^{3m}(dB+w_i/3)^p&\leq mB^p+9m(dB)^p+9m(dB+B/6)^p
\end{align*}
we have
\begin{align*}
    0&\geq \left(\sum_{i\in[3m],r\in[3]}w(\delta(X_i^r))^p+\sum_{j=1}^mw(\delta(S_j))^p-(mB^p+9m(dB)^p+9m(dB+B/6)^p)\right)B^{-p}
    \\&>|I|\big((d+1/6)^p-d^p-(1/4)^p\big)+9md^p+3m(1/4)^p-m-9m(d+1/6)^p
    \\&>|I|\big((d+1/6)^p-d^p-(1/4)^p\big)-m-(3/2)mp(d+1/6)^{p-1},
\end{align*}
where the last inequality follows from mean value theorem.
We note that due to mean value theorem, we also have
\begin{align*}
    (d+1/6)^p-d^p\geq pd^{p-1}/6=2^{p-1}\cdot p(m+1).
\end{align*}
This implies
\begin{align*}
    0>|I|\big((d+1/6)^p-d^p-(1/4)^p\big)-m-(3/2)mp(d+1/6)^{p-1},
\end{align*}
yielding a contradiction. Therefore, we must have $I=\emptyset$, proving our claim.

\end{proof}

To complete the backward direction, we need the following claim which derives a YES certificate for \textsc{3-partition} from an optimal multiway cut whose $\ell_p$ objective is at most $(9m(2dB)^p+mB^p)^{1/p}$.

\begin{claim}
Given an optimal multiway cut of $G$ whose $\ell_p$ objective is at most $(9m(2dB)^p+mB^p)^{1/p}$, let $S_j:=\{i\in[3m]:v_i\text{ is in the same part with }t_j\}$ for each $j\in[m]$. Then $S_1,S_2,\ldots,S_m$ together forms a partition of $S$ such that $\sum_{i\in S_j}w_i=B$ for each $j\in[m]$.
\end{claim}

\begin{proof}
Due the previous claim, we know that $S_1,\ldots,S_j$ must form a partition of $S$. This also implies that for each $i\in[3m]$, $r\in[3]$, $\{x_i^r\}$ is a part in the multiway cut. Therefore, we have
\begin{align*}
    9m(2dB)^p+mB^p&\geq \sum_{i\in[3m],r\in [3]}(2dB)^p+\sum_{j=1}^mw(\delta(S_j))^p
    =9m(2dB)^p+\sum_{j=1}^mw(\delta(S_j))^p.
\end{align*}
This implies $\sum_{j=1}^mw(\delta(S_j))^p\leq mB^p$. By H\"older's inequality, we observe that
\begin{align*}
    mB^p\geq\sum_{j=1}^mw(\delta(S_j))^p=\sum_{j=1}^m \left(\sum_{i\in S_j}w_i\right)^p\geq m\cdot\left(\frac{1}{m}\sum_{j=1}^m\sum_{i\in S_j}w_i\right)^p=mB^p.
\end{align*}
Here all inequalities are forced to be equations. This happens only when $\sum_{i\in S_j}w_i=B$ for all $j\in [m]$.
\end{proof}

With these three claims, we have derived a reduction from \textsc{3-partition} to min \lpnormmc for every fixed $p>1$. This finishes the proof of Theorem \ref{thm:NP-hard}.
